Self-Supervised Representations Improve End-to-End Speech Translation

End-to-end speech-to-text translation can provide a simpler and smaller system but is facing the challenge of data scarcity. Pre-training methods can leverage unlabeled data and have been shown to be effective on data-scarce settings. In this work, we explore whether self-supervised pre-trained speech representations can benefit the speech translation task in both high- and low-resource settings, whether they can transfer well to other languages, and whether they can be effectively combined with other common methods that help improve low-resource end-to-end speech translation such as using a pre-trained high-resource speech recognition system. We demonstrate that self-supervised pre-trained features can consistently improve the translation performance, and cross-lingual transfer allows to extend to a variety of languages without or with little tuning.

==> table_covo_ast.bak.tex <==
\begin{table*}[]
    \centering
    \caption{Comparison of different speech features for English ASR and X-to-En AST. The first column indicates the WER of EN ASR models used to pretrain the AST. The AST results are on CoVoST/Tatoeba test set (when available). The AST languages are: German (De), French (Fr), Spanish (Es), Dutch (Nl), Russian (Ru), Italian (It), Turkish (Tr), Persian (Fa), Swedish (Sv-SE), Mongolian (Mn) and Chinese (Zh-CN). The baseline \cite{wang2020covost} is comparable to the case with ASR encoder pre-training, using log-mel filterbank features.}
  \begin{adjustwidth}{-.4in}{-.5in}
        \begin{tabular}{c|c|cccccccccccc}
        \toprule
        Language & En & De & Fr & Es & Nl & Ru & It & Tr & Fa & Sv-SE & Mn & Zh-CN\\
        Hours (test) & & 168.3 & 46.3 & 3.5 & 8.2 & 8.2 & 12.8 & 3.8 & 23.9 & 1.0 & 2.9 & 3.7\\
        \midrule
        Wang et al. \cite{wang2020covost} & - & 7.6/7.5 & 21.4/10.9 & 6.1/1.9 & 3.4/5.0 & 4.8/1.1 & 6.5 & 3.1 & 2.8 & 1.9 & 0.3 & 5.6 \\
        \midrule
        \textbf{No ASR pre-training} \\
        fbank  &  & 3.08/1.45 & 17.27/6.37 & 0.84/0.49 & 0.11/0.14 & 1.3/0.07 & 0.46 & 1.13 & 0.29 & 0.17 & 0.36 & 2.44 \\
        wav2vec  &  & 6/\textbf{5.02} & \textbf{21.55/12.81} & 0.43/0.35 & 0.31/0.53 & \textbf{2.01}/0.07 & 0.44 & 0.94 & 1.58 & 0.26 & 0.18 & \textbf{3.47} \\
        vq-wav2vec  & & \textbf{6.08}/5.00 & 20.75/12.23 & 0.74/0.25 & 0.24/0.36 & 1.98/0.13 & 0.46 & 0.85 & 1.18 & 0.36 & 0.27 & 3 \\
        + BERT & & 2.75/1.24 & 18.36/7.39 & 0.18/0.15 & 0.11/0.15 & 1.42/0.07 & 0.4 & 0.55 & 0.22 & 0.27 & 0.13 & 2.83 \\\hdashline
        % BERT-backbone & \textbf{6.68}/ing & 16.41/ing & \textbf{3.37}/ing & \textbf{2.1}/ing & \textbf{5.05}/ing &  &  &  &  &  &  \\
        % \midrule
        BERT-backbone & & 6.68 & 16.41 & 3.37 & 2.1 & 5.05 &  &  &  &  &  &  \\
        \midrule
        \textbf{+ ASR enc} \\
        fbank & 34.32 & 7.15/6.59 & 21.86/10.3 & 5.48/1.93 & 3.25/3.94 & 5.06/0.83 & 6.99 & \textbf{3.44} & 2.65 & 1.82 & 0.16 & \textbf{6.92} \\
        wav2vec & 32.56 & \textbf{8.64/9.68} & \textbf{22.67/14.27} & \textbf{6.54/2.36} & 3.81/4.98 & \textbf{6.07/1.31} & \textbf{8.21} & 3.36 & 3.22 & \textbf{1.94} & 0.13 & 5.75 \\
        vq-wav2vec & 35 & 8.45/9.77 & 21.91/12.40 & \textbf{6.54/2.37} & 3.67/\textbf{5.43} & 5.72/1.25 & 7.84 & 3.07 & \textbf{3.27} & 1.75 & 0.33 & 5.66 \\
        + BERT & 32.05 & 7.62/8.33 & 19.69/10.42 & 5.74/2.39 & \textbf{4.20}/4.20 & 5.68/1.01 & 6.57 & 2.95 & 3.12 & 1.75 & 0.33 & 5.66 \\
        \midrule
        \textbf{+ ASR enc-dec} \\
        fbank &  & 8.28/7.4 & 22.50/11.22 & 6.82/2.20 & 4.00/5.48 & 8.33/1.35 & 8.84 & 3.17 & 3.09 & 2.97 & 0.21 & \textbf{8.15} \\
        wav2vec &  & \textbf{9.68}/10.12 & \textbf{23.02/14.33} & \textbf{7.17/3.63} & 4.86/6.86 & 8.82/\textbf{1.76} & \textbf{9.66} & \textbf{3.35} & \textbf{3.65} & \textbf{3.71} & 0.19 & 6.77 \\
        vq-wav2vec &  & 9.59/\textbf{11.19} & 22.05/13.05 & 6.89/3.29 & \textbf{4.95/7.03} & \textbf{9.19}/1.67 & 9.03 & 3.29 & \textbf{3.65} & 3.21 & 0.32 & 7.03 \\
        + BERT &  & 8.5/9.42 & 19.89/10.46 & 6.16/3.16 & 4.34/5.82 & 8.28/1.31 & 7.66 & 2.75 & 3.26 & 2.88 & 0.25 & 6.42 \\
        \bottomrule
        \end{tabular}
    \end{adjustwidth}
    \label{tab:table_covo_ast}
\end{table*}





==> table_covo_avg_per_group.tex <==
\begin{table*}[]
    \centering
    \caption{[TODO: reduce or remove the table] Average per-group mean and average coefficient of variation for ST sentence BLEU scores }
    \begin{tabular}{c|ccccccccccc|ccc}
    \toprule
        & \multicolumn{11}{c}{CoVoST} & \multicolumn{2}{c}{MuST-C} \\
        \midrule
        Language & de & fr & es & nl & ru & it & tr & fa & sv-SE & mn & zh-CN & en-fr & en-ro \\
        \midrule
        \textbf{No pretraining} & & & & & & & & & & & & & \\
        fbank & & & & & & & & & & & & & \\
        BLEU_{MS} & 1.33 & 9.617 & 0.259 & nl & ru & it & tr & 0.041 & sv-SE & mn & zh-CN & 22.549 & 11.485 \\
        CoefVar_{MS} & 2.562 & 0.801 & 1.454 & nl & ru & it & tr & 1.75 & sv-SE & mn & zh-CN & 0.428 & 0.816\\
        
        wav2vec & & & & & & & & & & & & & \\
        BLEU_{MS} & 2.617 & 13.214 & 0.109 & nl & ru & it & tr & 0.604 & sv-SE & mn & zh-CN & 24.31 & ing \\
        CoefVar_{MS} & 2.04 & 0.822 & 1.575 & nl & ru & it & tr & 1.304 & sv-SE & mn & zh-CN & 0.292 & ing \\
        
        vq-wav2vec & & & & & & & & & & & & & \\
        BLEU_{MS} & 2.634 & 12.469 & 0.19 & nl & ru & it & tr & 0.431 & sv-SE & mn & zh-CN & 23.373 & ing \\
        CoefVar_{MS} & 2.064 & 0.853 & 1.588 & nl & ru & it & tr & 1.336 & sv-SE & mn & zh-CN & 0.388 & ing \\

        + BERT & & & & & & & & & & & & & \\
        BLEU_{MS} & 1.225 & 10.036 & es & nl & ru & it & tr & 0.034 & sv-SE & mn & zh-CN & 23.358 & ing \\
        CoefVar_{MS} & 2.445 & 0.889 & es & nl & ru & it & tr & 2.175 & sv-SE & mn & zh-CN & 0.387 & ing \\
        \midrule
        
        \textbf{+ ASR enc} & & & & & & & & & & & & & \\
        fbank & & & & & & & & & & & & & \\
        BLEU_{MS} & 3.113 & 13.655 & 0.034 & nl & ru & it & tr & 1.285 & sv-SE & mn & zh-CN &  & \\
        CoefVar_{MS} & 2.133 & 0.745 & 1.626 & nl & ru & it & tr & 1.275 & sv-SE & mn & zh-CN & &  & \\
        
        wav2vec & & & & & & & & & & & & & \\
        BLEU_{MS} & 3.571 & 14.408 & es & nl & ru & it & tr & 1.549 & sv-SE & mn & zh-CN & &  & \\
        CoefVar_{MS} & 2.123 & 0.785 & es & nl & ru & it & tr & 1.391 & sv-SE & mn & zh-CN &  & \\
        
        vq-wav2vec & & & & & & & & & & & & & \\
        BLEU_{MS} & 3.843 & 13.645 & es & nl & ru & it & tr & 1.635 & sv-SE & mn & zh-CN &  & \\
        CoefVar_{MS} & 2.161 & 0.81 & es & nl & ru & it & tr & 1.442 & sv-SE & mn & zh-CN &  & \\

        + BERT & & & & & & & & & & & & & \\
        BLEU_{MS} & 3.369 & 11.729 & es & nl & ru & it & tr & 1.516 & sv-SE & mn & zh-CN &  & \\
        CoefVar_{MS} & 2.248 & 0.861 & es & nl & ru & it & tr & 1.344 & sv-SE & mn & zh-CN &  & \\
        
        \midrule
        \textbf{+ ASR enc-dec} & & & & & & & & & & & & & \\
        fbank & & & & & & & & & & & & & \\
        BLEU_{MS} & de & fr & es & nl & ru & it & tr & 1.285 & sv-SE & mn & zh-CN & - & - \\
        CoefVar_{MS} & de & fr & es & nl & ru & it & tr & 1.285 & sv-SE & mn & zh-CN & - & -\\
        
        wav2vec & & & & & & & & & & & & & \\
        BLEU_{MS} & de & fr & es & nl & ru & it & tr & 1.285 & sv-SE & mn & zh-CN & - & - \\
        CoefVar_{MS} & de & fr & es & nl & ru & it & tr & 1.285 & sv-SE & mn & zh-CN & - & - \\
        
        vq-wav2vec & & & & & & & & & & & & & \\
        BLEU_{MS} & de & fr & es & nl & ru & it & tr & 1.285 & sv-SE & mn & zh-CN & - & - \\
        CoefVar_{MS} & de & fr & es & nl & ru & it & tr & 1.285 & sv-SE & mn & zh-CN & - & - \\

        + BERT & & & & & & & & & & & & & \\
        BLEU_{MS} & de & fr & es & nl & ru & it & tr & 1.285 & sv-SE & mn & zh-CN & - & - \\
        CoefVar_{MS} & de & fr & es & nl & ru & it & tr & 1.285 & sv-SE & mn & zh-CN & - & - \\
    \bottomrule
    \end{tabular}
    \label{tab:coefvar}
\end{table*}

==> table_covo_specaugment.tex <==
\begin{table*}[th]
\begin{adjustwidth}{-.4in}{-.5in}
    \centering
    \caption{[TODO: Will remove the table (comment in the paper added) - slight improvement on high-res only] No SpecAugment}
    \begin{tabular}{c|cccccccccccc}
    \toprule
        Language & de & fr & es & nl & ru & it & tr & fa & sv-SE & mn & zh-CN\\
        Hours (test) & de & fr & es & nl & ru & it & tr & fa & sv-SE & mn & zh-CN\\
        \midrule
        Wang et al. \cite{wang2020covost} & 7.6/7.5 & 21.4/10.9 & 6.1/1.9 & 3.4/5.0 & 4.8/1.1 & 6.5 & 3.1 & 2.8 & 1.9 & 0.3 & 5.6 \\
        \midrule
        \textbf{No pretraining} \\
        fbank  & 3.40/1.73 & 16.62/7.09 & 0.60/0.18 & 0.45/1.18 & 1.77/0.05 & 0.59 & 1.22 & 0.41 & 0.20 & 0.18 & 3.14\\
        wav2vec  & 6.09/4.60 & 20.27/11.92 & 1.06/0.42 & 0.09/0.66 & 2.40/0.09 & 0.44 & tr & 1.86 & 0.40 & 0.19 & 3.47\\
        vq-wav2vec  & 6.04/4.68 & 19.72/11.92 & 0.69/0.32 & 0.80/2.71 & 1.95/0.12 & 0.39 & 0.74 & fa & 0.67 & 0.15 & 3.00\\
        + BERT & 2.72/1.16 & 17.35/7.50 & 0.11/0.21 & 0.10/0.23 & 1.37/0.08 & it & 0.49 & 0.15 & 0.26 & 0.15 & 2.78\\
        \bottomrule
    \end{tabular}
    \end{adjustwidth}
    \label{tab:covo}
\end{table*}{}
